Fast and simple unrooted dynamic forests

A dynamic forest data structure maintains a forest (and associated data like edge weights) under edge insertions and deletions. Dynamic forests are widely used to solve online and offline graph problems. Well-known examples of dynamic forest data structures are link-cut trees [Sleator and Tarjan '83] and top trees [Alstrup, Holm, de Lichtenberg, and Thorup '05], both of which need O(log n) time per operation. While top trees are more flexible and arguably easier to use, link-cut trees are faster in practice [Tarjan and Werneck '10]. In this paper, we propose an alternative to link-cut trees. Our data structure is based on search trees on trees (STTs, also known as elimination trees) and an STT algorithm [Berendsohn and Kozma '22] based on the classical Splay trees [Sleator and Tarjan '85]. While link-cut trees maintain a hierarchy of binary search trees, we maintain a single STT. Most of the complexity of our data structure lies in the implementation of the STT rotation primitive, which can easily be reused, simplifying the development of new STT-based approaches. We implement several variants of our data structure in the Rust programming language, along with an implementation of link-cut trees for comparison. Experimental evaluation suggests that our algorithms are faster when the dynamic forest is unrooted, while link-cut trees are faster for rooted dynamic forests.

==> figures/table_num_rotations.tex <==
	\begin{tabular}{lccccc}
		\toprule
		& \multicolumn{5}{c}{
Number of rotations/query}\\		\cmidrule{2-6}Algorithm & $n = 1000$ & $n = 2000$ & $n = 3000$ & $n = 4000$ & $n = 5000$\\
		\midrule
		Greedy Splay & $9.659$ & $10.530$ & $11.277$ & $11.643$ & $12.090$\\
		2P Splay & $9.202$ & $10.094$ & $10.820$ & $11.196$ & $11.625$\\
		L2P Splay & $9.290$ & $10.137$ & $10.865$ & $11.224$ & $11.662$\\
		MTR & $9.588$ & $10.430$ & $11.172$ & $11.527$ & $11.971$\\
		\bottomrule
	\end{tabular}


==> figures/table_uniform.tex <==
	\begin{tabular}{lcc}
		\toprule
		& \multicolumn{2}{c}{
Running time (\textmu{}s/query)}\\		\cmidrule{2-3}Algorithm & $n = 500$ & $n = 1000$\\
		\midrule
		Petgraph & $3.87$ & $7.64$\\
		Link-cut & $0.45$ & $0.48$\\
		Greedy Splay & $0.36$ & $0.39$\\
		Stable Greedy Splay & $0.34$ & $0.36$\\
		2P Splay & $0.40$ & $0.41$\\
		Stable 2P Splay & $0.35$ & $0.37$\\
		L2P Splay & $0.33$ & $0.38$\\
		Stable L2P Splay & $0.31$ & $0.36$\\
		MTR & $0.29$ & $0.32$\\
		Stable MTR & $0.27$ & $0.31$\\
		1-cut & $0.10$ & $0.16$\\
		\bottomrule
	\end{tabular}

